Scalable Qubit Representations of Neutrino Mixing Matrices

Oscillating neutrino beams exhibit quantum coherence over distances of thousands of kilometers. Their unambiguously quantum nature suggests an appealing test system for direct quantum simulation. Such techniques may enable presently analytically intractable calculations involving multi-neutrino entanglements, such as collective neutrino oscillations in supernovae, but only once oscillation phenomenology is properly re-expressed in the language of quantum circuits. Here we resolve outstanding conceptual issues regarding encoding of arbitrarily mixed neutrino flavor states in the Hilbert space of an n-qubit quantum computer. We introduce algorithms to encode mixing and oscillation of any number of flavor-mixed neutrinos, both with and without CP-violation, with an efficient number of prescriptive input parameters in terms of sub-rotations of the PMNS matrix in standard form. Examples encoded for an IBM-Q quantum computer are shown to converge to analytic predictions both with and without CP-violation.

==> newfig.tex <==
(I wasn't sure how to implement this in your figure, but here's the circuit expresion for R23 that you asked for:) 

$$\scalebox{1.0}{
\Qcircuit @C=1.0em @R=0.2em @!R { \\
	 	\nghost{ {q}_{0} :  } & \lstick{ {q}_{0} :  } & \ctrlo{1} & \qswap & \ctrlo{1} & \qswap & \ctrlo{1} & \qw & \qw\\ 
	 	\nghost{ {q}_{1} :  } & \lstick{ {q}_{1} :  } & \targ & \qswap \qwx[-1] & \gate{\mathrm{U_3}\,(\mathrm{-2\theta,-\delta,\delta})} & \qswap \qwx[-1] & \targ & \qw & \qw\\ 
\\ }}}$$

